Architectures for Heterogeneous Quantum Error Correction Codes

Quantum Error Correction (QEC) is essential for future quantum computers due to its ability to exponentially suppress physical errors. The surface code is a leading error-correcting code candidate because of its local topological structure, experimentally achievable thresholds, and support for universal gate operations with magic states. However, its physical overhead scales quadratically with number of correctable errors. Conversely, quantum low-density parity-check (qLDPC) codes offer superior scaling but lack, on their own, a clear path to universal logical computation. Therefore, it is becoming increasingly evident is becoming that there are significant advantages to designing architectures using multiple codes. Heterogeneous architectures provide a clear path to universal logical computation as well as the ability to access different resource trade offs. To address this, we propose integrating the surface code and gross code using an ancilla bus for inter-code data movement. This approach involves managing trade-offs, including qubit overhead, a constrained instruction set, and gross code (memory) routing and management. While our focus is on the gross-surface code architecture, our method is adaptable to any code combination and the constraints generated by that specific architecture. Motivated by the potential reduction of physical qubit overhead, an ever important feature in the realization of fault tolerant computation, we perform the first full system study of heterogeneous error-correcting codes, discovering architectural trade-offs and optimizing around them. We demonstrate physical qubit reductions of up to 6.42x when executing an algorithm to a specific logical error rate, at the cost of up to a 3.43x increase in execution time.

==> text/modeling.tex <==
\section{Modeling(Shifan's notes)}

In summary, the following contents in this section will be:
\begin{enumerate}
    \item A instruction set of Heterogeneous QEC architecture, which maps logical circuits into Hetec instructions, with detailed cost of physical implementation for every logical operation.
    \item A two-level fault tolerant compiler, which consists of an instruction transpiler and physical gate synthesizer. The former transpires a Clifford+T circuit into the Pauli-based computation gates, with fetching and storing between Surface blocks and QLDPC blocks (in the instructions set), and the latter further generates Hetec instructions with physical gates executable in hardware.
    \item A circuit fidelity estimator. Taking the transpiled circuit, the fidelity estimator automatically computes an estimated fidelity of the circuit executed in such Hetec architecture. The estimator's accuracy can be further improved by more fine-grained simulation to access the error model after applying the logical gate.
\end{enumerate}


% \subsubsection{QLDPC instructions}

% All the qubits in the gross code can be described by two types L or R and a set of mononials $\mathcal{M}$, where $\mathcal{M}=\{ 1,x,...,x^l,xy,...x^ly,...,x^ly^m\}$, with $l=12, m=6$. Combining the two will give a unique label to any individual qubits in the QLDPC block. The logical Pauli X/Z operators supported by physical qubits are described by subsets of monomials, and the choices can be different, as long as the selected subsets could span the entire logical qubit space. Here, we propose two possible selections of logical operators:
% \begin{enumerate}
%     \item Selection 1: 
%     \begin{align}
% \bar{X}_\alpha & :=X(\alpha f, 0) & \bar{Z}_\beta & :=Z\left(\beta h^T, \beta g^T\right) \\
% \bar{X}_\alpha^{\prime} & :=X(\alpha g, \alpha h) & \bar{Z}_\beta^{\prime} & :=Z\left(0, \beta f^T\right)
%     \end{align}
% Where $f,g,h$ is a pre-determined subset of group $\mathcal{M}$, and $\alpha=\{1, y, x^2y, x^2y^5, x^3y^2, x^4\}$, $\beta=\{y, y^5, xy, 1, x^4, x^5y^2\}$. Notice the X and Z operators are using prefactor, i.e., sets of $\alpha$ and $\beta$ are different. This increases the overhead of measuring logical qubits in QLDPC and applying logical operators, which requires both X and Z measurements. The prefactor now is "unsynced" and needs to be treated separately.
    
% Also, notice in this choice that the logical Pauli X gate is only associated with the L data qubits, which avoids a crossing ancilla system between L and R data qubits.
    
%     \item Selection 2:
%     \begin{align}
% \bar{X} & :=X(\gamma p, \gamma q) & \bar{Z} & :=Z\left(\gamma r, \gamma s\right) \\
% \bar{X}_\gamma^{\prime} & :=X(\gamma s^T, \gamma r^T) & \bar{Z}_\gamma^{\prime} & :=Z\left(\gamma q^T, \gamma p^T\right)
%     \end{align}

%     This selection allows the logical operator to be supported both on L and R qubits. More importantly, it eliminates the requirement of separated parameters $\alpha$ and $\beta$, with a unified parameter $\gamma$ to indicate pairs of logical operators. This could bring convenience regarding tracking logical qubits and synthesizing automorphism gates, as the X and Z operators will be shifted "synchronously" by applying automorphism gates.
% \end{enumerate}

% Automorphism gates provide the ability to implement fault-tolerant in-block permutation of logical qubits. Such gates utilize the connectivity of checker qubits and data qubits, implementing fault-tolerant data qubits permutation. The operations could be described using the generators of the parity checker matrix H.

% In gross code, the possible automorphism operation could be described in the form of $A_iA_j^T$ or $B_iB_j^T$, which serves as the generator set $ \omega=\{x,x^2,x^4,x^5,xy,..,\}$.( $A_i= \{x^3,y,y^2\}, B_i= \{y^3,x,x^2\})$. This means we could \emph{synthesis} the Pauli operator choices in the above using this generator set. We will elaborate more details on automorphism gates in the section on ancilla operations.

% ZX duality gates allow switching supporting qubits of logical X and logical Z operators, hence fetching logical qubits in the prime block without introducing more ancillary qubits attached to the $m_i$ set. In particular, the operations are still using the connectivity defined by matrices $A$ and $B$ to swap $X_\alpha=X(\alpha f,0)$ with Z $\alpha^T = Z(0,\alpha^T f^T)$, as well as $Z_\alpha=Z(\alpha h^T,\alpha g^T)$ with $X_\alpha=X(\alpha g,\alpha h)$.

% However, such gates require a very long-depth gate sequence of up to 132 CNOTs. We assume the physical error rate fidelity is 132 times worse than the original gate and figure out the logical error rate of this operation. As shown in the table, the physical error rate exceeds the threshold of the gross code, and we suggest not applying the ZX duality gate by trading half of the logical qubit capacity. As such, we will not use the logical qubits from the primed block.

\subsection{Instructions in Heterogeneous QEC architecture}


\subsection{Circuit fidelity estimator}
Based on the instructions defined above, it is possible to give an estimated circuit fidelity when executed in such a heterogeneous architecture. This is achieved by a two-level error rate simulation protocol, where we simulate the logical error rate in every logical operator, then substitute the original circuit with instructions and simulate again. The estimator could be further improved by not only simulating the logical error rate for every instruction but also the full error model before and after the physical gates for instructions are applied. 


We provide a universal instruction set in Heterogeneous QEC architecture, which ensures universal computation for any quantum circuits. It consists of three types of instructions: Surface code, QLDPC, and ancilla, which intuitively refer to operations involving surface code only, QLDPC code only, and joint operation on ancillary qubits.



\subsection{Notes}
Logical clock rate

Ratio of qubit in qldpc and surface, what is the sweet point for different algorithms

Logical error rate graph


\subsubsection{Ancilla instructions}
Ancilla system serves as a core component in the Hetec system, as it implements the function of logical operator measurement, which is also used to teleport logical qubits between the surface patch and the QLDPC blocks. Specifically, we consider both CKBB, SSIP and the mono-layer scheme. The former is considered general enough but costly for joint X measurement of arbitrary CSS codes, while the mono-layer is resource-efficient but hasn't been constructed to the code, and SSIP is between the two.

Basically, the ancilla system will serve as shown in Figure~\ref{fig:qubitm}; when attached to X or Z logical operators, the ancilla system is able to implement bi-directional CNOT gates, which is a similar scheme of measurement-based CNOT used in surface code lattice surgery.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\linewidth]{figs/teleport.pdf}
    \caption{Moving qubit between blocks by joint XX measurement}
            \label{fig:teleport}
\end{figure}

The ancilla system is manufactured to be attached to a ``probe'' qubit, with the monomial label, e.g., ``1''. Any other qubits, whenever requested, will go through several rounds of automorphism gate to be fetched. Algorithm~\ref{alg:fetch} described the detailed steps of the fetching operation from QLDPC to the surface block.

\begin{algorithm}[h]
\caption{Fetching the qubits from QLDPC block}\label{alg:fetch}
\begin{algorithmic}[1]

\State \textbf{Require: } Current probe qubit monomial $m_{X_p}$ and $m_{Z_p}$
\State \textbf{Require: } Target qubit monomial $m_{X_t}$ and $m_{Z_p}$ 
\State \textbf{Require: } Operator set $ \omega=\{x,x^2,x^4,x^5,xy,..,\}$

\State Compute differential $m_d=m_{X_t}/m_{Xsc_p}$
\State Find the minimum rounds of automorphism gates as a sequence of valid operations in the set $OP$, denoted as $m_d=\omega_1\omega_2...$, where$\omega_i \in OP$, the length of the sequence decides the rounds of the automorphism gates required.
\State Apply XX measurement using ancilla block.
\State Compute differential $m_d'=(m_{Z_t}/m_{Z_p})/m_d$.
\Comment{Note in synced choice of Pauli operators, $m_d'$ is always 1}
\State Find the minimum rounds of automorphism gates as a sequence of valid operations in the set $OP$.
\State Apply Z measurement in QLDPC block.
\State Apply classical correction to Surface code according to previous two measurement outcomes.
\State Update the probe qubit to the current monomial $m_{X_t}$ and $m_{Z_p}$
\end{algorithmic}
\end{algorithm}
Notice in the logical operation selection 2 that the X and Z operators can be shifted with the same monomial $\gamma$; hence, for every store/fetch operation, only X logical operator automorphism gates are required. However, when X and Z operators are shifted with the different monomial $\alpha$ and $\beta$, the store and fetch will be slightly more complex, each synthesizing X,Z. Specifically, it goes through the following operations: automorphism gate $\alpha$, which swaps probe qubit X with target qubit X, followed by automorphism $\beta/\alpha$, which swaps the physical qubit undergo $\alpha$ to the target Z. 

We summarize the above description and detailed parameters of the gates in Table~\ref{tab:QLDPCinst}.


\begin{table*}[t]
    \centering
    \begin{tabular}{ p{3.6cm}||p{2cm}|p{2.6cm}|p{4cm}|p{4cm}}
     \hline
     \hline
       Operations & Ancillary qubits & Circuit Depth & Logical error probability & Notes \\
     \hline
     Pauli operators & null & 1 gate time  (parallelism 12) & $10^{-7}$ & \\
     \hline
     Automorphism & null & 2 * two-qubit gate time * steps (Figure~\ref{fig:step}) & $10^{-7}$ &   \\
     \hline
     ZX-duality & null & 132 CNOT depth & Not-fault-tolerant & $132p$ gives an physical error rate higher than the threshold of the code  \\
     \hline
     Measurement-based CNOT[CKBB]&  $1380$ &  12 rounds of syndrome measurement + decoder time + automorphism gates (routing overhead) & $10^{-3}$ from Qian Xu &  \\
     \hline
     Measurement-based CNOT[SSIP]&  $180$ &  12 rounds of syndrome measurement + decoder time + automorphism gates (routing overhead) & no-simulation results&  \\
     \hline
     Measurement-based CNOT[mono-layer]&  $103$ & 7 rounds of syndrome measurement+ decoder time + automorphism gates (routing overhead) & $ 9* 10^{-5}$& Not sure if works for BB+Surface \\
    \end{tabular}
    \caption{Instructions in BB code with estimated error probability, assuming physical error rate $p=10^{-3}$, where single-qubit Pauli gate and CNOT gate error same as physical error rate. We also assume syndrome measurement and decoding after each logical operation.}
    \label{tab:QLDPCinst}
\end{table*}

\begin{table*}[t]
    \centering
    \begin{tabular}{ p{3.6cm}||p{2cm}|p{2.6cm}|p{4cm}|p{4cm}}
     \hline
     \hline
       Operations & $p=10^{-5}$ Fit by BCG24 & $p=10^{-4}$ & $p=10^{-3}$ & Notes \\
     \hline
     Pauli operators & $10^{-17}$ & $10^{-12}$ & $10^{-7}$ & \\
     \hline
     Automorphism & $10^{-17}$ & $10^{-12}$ & $10^{-7}$ &   \\
     \hline
     ZX-duality & $5*10^{-6}$ & Not-fault-tolerant & Not-fault-tolerant & $132p$ gives a physical error rate higher than the threshold of the code  \\
     \hline
     Measurement-based CNOT[CKBB]&  no-simulation results &  no-simulation results & $10^{-3}$ from Qian Xu &  \\
     \hline
     Measurement-based CNOT[SSIP]&  no-simulation results &  no-simulation results & no-simulation results&  \\
     \hline
     Measurement-based CNOT[mono-layer]&  $ 3*10^{-17}$ & $ 6* 10^{-12}$ & $ 9* 10^{-5}$& Not sure if works for BB+Surface \\
    \end{tabular}
    \caption{Instructions in BB code with estimated error probability, assuming physical error rate $p=10^{-3}$, where single-qubit Pauli gate and CNOT gate error same as physical error rate. We also assume syndrome measurement and decoding after each logical operation.}
    \label{tab:QLDPCinst2}
\end{table*}


\begin{table*}[t]
    \centering
    \begin{tabular}{ p{3.6cm}||p{2cm}|p{2.6cm}|p{4cm}|p{4cm}}
     \hline
     \hline
       Operations & Ancillary qubits & Circuit Depth & Logical error probability & logical clock rate \\
     \hline
     Pauli operators & null & 1 gate time (parallelism 12) & idling error $10^{-7}$ &  \\
     \hline
     magic state  & null & varied gate time& idling error $10^{-7}$ &  \\
     \hline
    \end{tabular}
    \caption{Instructions in surface code with estimated error probability, assuming physical error rate $p=10^{-3}$.}
    \label{tab:surinst}
\end{table*}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figs/adjmatrix.pdf}
    \caption{Automorphism rounds required between the movement of logical qubits X/Z}
            \label{fig:adjmatrix}
\end{figure}

\subsection{Logical qubit mapper and Fault-tolerant compiler}
We will need to design a logical qubit mapper in the circuits. Based on the DAG, we need to track if a qubit is in Memory, where in Memory, or where in Surface code. Notice that this could be high, but in this work, we will \textbf{not} focus on the routing optimization problem. 

Instead, we assume the ancillary block is linked to the first logical qubit, labeled as $k=0$ ($\alpha=0$), where $k$ is a logical qubit label and $\alpha$ is the monomial corresponding to 

As introduced in the ancilla instructions, the fault-tolerant compiler could generate the minimum-round automorphism operations required for a specific permutation of physical qubits. The logical qubit mapper then will update the index of each logical qubit according to every automorphism/ZX duality gate is applied, and synthesize next-round automorphism gates according to the current logical qubit distribution topology.

The number of automorphism gates needed in the gross code are numerically searched and listed in Figure~\ref{fig:stepx} and Figure~\ref{fig:stepz}.


\subsubsection{Ancilla instructions}
Ancilla system serves as a core component in the Hetec system, as it implements the function of logical operator measurement, which is also used to teleport logical qubits between the surface patch and the QLDPC blocks. Specifically, we consider both CKBB, SSIP and the mono-layer scheme. The former is considered general enough but costly for joint X measurement of arbitrary CSS codes, while the mono-layer is resource-efficient but hasn't been constructed to the code, and SSIP is between the two.

Basically, the ancilla system will serve as shown in Figure~\ref{fig:qubitm}; when attached to X or Z logical operators, the ancilla system is able to implement bi-directional CNOT gates, which is a similar scheme of measurement-based CNOT used in surface code lattice surgery.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\linewidth]{figs/teleport.pdf}
    \caption{Moving qubit between blocks by joint XX measurement}
            \label{fig:teleport}
\end{figure}

The ancilla system is manufactured to be attached to a ``probe'' qubit, with the monomial label, e.g., ``1''. Any other qubits, whenever requested, will go through several rounds of automorphism gate to be fetched. Algorithm~\ref{alg:fetch} described the detailed steps of the fetching operation from QLDPC to the surface block.

\begin{algorithm}[h]
\caption{Fetching the qubits from QLDPC block}\label{alg:fetch}
\begin{algorithmic}[1]

\State \textbf{Require: } Current probe qubit monomial $m_{X_p}$ and $m_{Z_p}$
\State \textbf{Require: } Target qubit monomial $m_{X_t}$ and $m_{Z_p}$ 
\State \textbf{Require: } Operator set $ \omega=\{x,x^2,x^4,x^5,xy,..,\}$

\State Compute differential $m_d=m_{X_t}/m_{Xsc_p}$
\State Find the minimum rounds of automorphism gates as a sequence of valid operations in the set $OP$, denoted as $m_d=\omega_1\omega_2...$, where$\omega_i \in OP$, the length of the sequence decides the rounds of the automorphism gates required.
\State Apply XX measurement using ancilla block.
\State Compute differential $m_d'=(m_{Z_t}/m_{Z_p})/m_d$.
\Comment{Note in synced choice of Pauli operators, $m_d'$ is always 1}
\State Find the minimum rounds of automorphism gates as a sequence of valid operations in the set $OP$.
\State Apply Z measurement in QLDPC block.
\State Apply classical correction to Surface code according to previous two measurement outcomes.
\State Update the probe qubit to the current monomial $m_{X_t}$ and $m_{Z_p}$
\end{algorithmic}
\end{algorithm}
Notice in the logical operation selection 2 that the X and Z operators can be shifted with the same monomial $\gamma$; hence, for every store/fetch operation, only X logical operator automorphism gates are required. However, when X and Z operators are shifted with the different monomial $\alpha$ and $\beta$, the store and fetch will be slightly more complex, each synthesizing X,Z. Specifically, it goes through the following operations: automorphism gate $\alpha$, which swaps probe qubit X with target qubit X, followed by automorphism $\beta/\alpha$, which swaps the physical qubit undergo $\alpha$ to the target Z. 

We summarize the above description and detailed parameters of the gates in Table~\ref{tab:QLDPCinst}.


\begin{table*}[t]
    \centering
    \begin{tabular}{ p{3.6cm}||p{2cm}|p{2.6cm}|p{4cm}|p{4cm}}
     \hline
     \hline
       Operations & Ancillary qubits & Circuit Depth & Logical error probability & Notes \\
     \hline
     Pauli operators & null & 1 gate time  (parallelism 12) & $10^{-7}$ & \\
     \hline
     Automorphism & null & 2 * two-qubit gate time * steps (Figure~\ref{fig:step}) & $10^{-7}$ &   \\
     \hline
     ZX-duality & null & 132 CNOT depth & Not-fault-tolerant & $132p$ gives an physical error rate higher than the threshold of the code  \\
     \hline
     Measurement-based CNOT[CKBB]&  $1380$ &  12 rounds of syndrome measurement + decoder time + automorphism gates (routing overhead) & $10^{-3}$ from Qian Xu &  \\
     \hline
     Measurement-based CNOT[SSIP]&  $180$ &  12 rounds of syndrome measurement + decoder time + automorphism gates (routing overhead) & no-simulation results&  \\
     \hline
     Measurement-based CNOT[mono-layer]&  $103$ & 7 rounds of syndrome measurement+ decoder time + automorphism gates (routing overhead) & $ 9* 10^{-5}$& Not sure if works for BB+Surface \\
    \end{tabular}
    \caption{Instructions in BB code with estimated error probability, assuming physical error rate $p=10^{-3}$, where single-qubit Pauli gate and CNOT gate error same as physical error rate. We also assume syndrome measurement and decoding after each logical operation.}
    \label{tab:QLDPCinst}
\end{table*}

\begin{table*}[t]
    \centering
    \begin{tabular}{ p{3.6cm}||p{2cm}|p{2.6cm}|p{4cm}|p{4cm}}
     \hline
     \hline
       Operations & $p=10^{-5}$ Fit by BCG24 & $p=10^{-4}$ & $p=10^{-3}$ & Notes \\
     \hline
     Pauli operators & $10^{-17}$ & $10^{-12}$ & $10^{-7}$ & \\
     \hline
     Automorphism & $10^{-17}$ & $10^{-12}$ & $10^{-7}$ &   \\
     \hline
     ZX-duality & $5*10^{-6}$ & Not-fault-tolerant & Not-fault-tolerant & $132p$ gives a physical error rate higher than the threshold of the code  \\
     \hline
     Measurement-based CNOT[CKBB]&  no-simulation results &  no-simulation results & $10^{-3}$ from Qian Xu &  \\
     \hline
     Measurement-based CNOT[SSIP]&  no-simulation results &  no-simulation results & no-simulation results&  \\
     \hline
     Measurement-based CNOT[mono-layer]&  $ 3*10^{-17}$ & $ 6* 10^{-12}$ & $ 9* 10^{-5}$& Not sure if works for BB+Surface \\
    \end{tabular}
    \caption{Instructions in BB code with estimated error probability, assuming physical error rate $p=10^{-3}$, where single-qubit Pauli gate and CNOT gate error same as physical error rate. We also assume syndrome measurement and decoding after each logical operation.}
    \label{tab:QLDPCinst2}
\end{table*}


\begin{table*}[t]
    \centering
    \begin{tabular}{ p{3.6cm}||p{2cm}|p{2.6cm}|p{4cm}|p{4cm}}
     \hline
     \hline
       Operations & Ancillary qubits & Circuit Depth & Logical error probability & logical clock rate \\
     \hline
     Pauli operators & null & 1 gate time (parallelism 12) & idling error $10^{-7}$ &  \\
     \hline
     magic state  & null & varied gate time& idling error $10^{-7}$ &  \\
     \hline
    \end{tabular}
    \caption{Instructions in surface code with estimated error probability, assuming physical error rate $p=10^{-3}$.}
    \label{tab:surinst}
\end{table*}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figs/adjmatrix.pdf}
    \caption{Automorphism rounds required between the movement of logical qubits X/Z}
            \label{fig:adjmatrix}
\end{figure}

\subsection{Logical qubit mapper and Fault-tolerant compiler}
We will need to design a logical qubit mapper in the circuits. Based on the DAG, we need to track if a qubit is in Memory, where in Memory, or where in Surface code. Notice that this could be high, but in this work, we will \textbf{not} focus on the routing optimization problem. 

Instead, we assume the ancillary block is linked to the first logical qubit, labeled as $k=0$ ($\alpha=0$), where $k$ is a logical qubit label and $\alpha$ is the monomial corresponding to 

As introduced in the ancilla instructions, the fault-tolerant compiler could generate the minimum-round automorphism operations required for a specific permutation of physical qubits. The logical qubit mapper then will update the index of each logical qubit according to every automorphism/ZX duality gate is applied, and synthesize next-round automorphism gates according to the current logical qubit distribution topology.

The number of automorphism gates needed in the gross code are numerically searched and listed in Figure~\ref{fig:stepx} and Figure~\ref{fig:stepz}.

\subsubsection{Ancilla instructions}
Ancilla system serves as a core component in the Hetec system, as it implements the function of logical operator measurement, which is also used to teleport logical qubits between the surface patch and the QLDPC blocks. Specifically, we consider both CKBB, SSIP and the mono-layer scheme. The former is considered general enough but costly for joint X measurement of arbitrary CSS codes, while the mono-layer is resource-efficient but hasn't been constructed to the code, and SSIP is between the two.

Basically, the ancilla system will serve as shown in Figure~\ref{fig:qubitm}; when attached to X or Z logical operators, the ancilla system is able to implement bi-directional CNOT gates, which is a similar scheme of measurement-based CNOT used in surface code lattice surgery.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\linewidth]{figs/teleport.pdf}
    \caption{Moving qubit between blocks by joint XX measurement}
            \label{fig:teleport}
\end{figure}

The ancilla system is manufactured to be attached to a ``probe'' qubit, with the monomial label, e.g., ``1''. Any other qubits, whenever requested, will go through several rounds of automorphism gate to be fetched. Algorithm~\ref{alg:fetch} described the detailed steps of the fetching operation from QLDPC to the surface block.

\begin{algorithm}[h]
\caption{Fetching the qubits from QLDPC block}\label{alg:fetch}
\begin{algorithmic}[1]

\State \textbf{Require: } Current probe qubit monomial $m_{X_p}$ and $m_{Z_p}$
\State \textbf{Require: } Target qubit monomial $m_{X_t}$ and $m_{Z_p}$ 
\State \textbf{Require: } Operator set $ \omega=\{x,x^2,x^4,x^5,xy,..,\}$

\State Compute differential $m_d=m_{X_t}/m_{Xsc_p}$
\State Find the minimum rounds of automorphism gates as a sequence of valid operations in the set $OP$, denoted as $m_d=\omega_1\omega_2...$, where$\omega_i \in OP$, the length of the sequence decides the rounds of the automorphism gates required.
\State Apply XX measurement using ancilla block.
\State Compute differential $m_d'=(m_{Z_t}/m_{Z_p})/m_d$.
\Comment{Note in synced choice of Pauli operators, $m_d'$ is always 1}
\State Find the minimum rounds of automorphism gates as a sequence of valid operations in the set $OP$.
\State Apply Z measurement in QLDPC block.
\State Apply classical correction to Surface code according to previous two measurement outcomes.
\State Update the probe qubit to the current monomial $m_{X_t}$ and $m_{Z_p}$
\end{algorithmic}
\end{algorithm}
Notice in the logical operation selection 2 that the X and Z operators can be shifted with the same monomial $\gamma$; hence, for every store/fetch operation, only X logical operator automorphism gates are required. However, when X and Z operators are shifted with the different monomial $\alpha$ and $\beta$, the store and fetch will be slightly more complex, each synthesizing X,Z. Specifically, it goes through the following operations: automorphism gate $\alpha$, which swaps probe qubit X with target qubit X, followed by automorphism $\beta/\alpha$, which swaps the physical qubit undergo $\alpha$ to the target Z. 

We summarize the above description and detailed parameters of the gates in Table~\ref{tab:QLDPCinst}.


\begin{table*}[t]
    \centering
    \begin{tabular}{ p{3.6cm}||p{2cm}|p{2.6cm}|p{4cm}|p{4cm}}
     \hline
     \hline
       Operations & Ancillary qubits & Circuit Depth & Logical error probability & Notes \\
     \hline
     Pauli operators & null & 1 gate time  (parallelism 12) & $10^{-7}$ & \\
     \hline
     Automorphism & null & 2 * two-qubit gate time * steps (Figure~\ref{fig:step}) & $10^{-7}$ &   \\
     \hline
     ZX-duality & null & 132 CNOT depth & Not-fault-tolerant & $132p$ gives an physical error rate higher than the threshold of the code  \\
     \hline
     Measurement-based CNOT[CKBB]&  $1380$ &  12 rounds of syndrome measurement + decoder time + automorphism gates (routing overhead) & $10^{-3}$ from Qian Xu &  \\
     \hline
     Measurement-based CNOT[SSIP]&  $180$ &  12 rounds of syndrome measurement + decoder time + automorphism gates (routing overhead) & no-simulation results&  \\
     \hline
     Measurement-based CNOT[mono-layer]&  $103$ & 7 rounds of syndrome measurement+ decoder time + automorphism gates (routing overhead) & $ 9* 10^{-5}$& Not sure if works for BB+Surface \\
    \end{tabular}
    \caption{Instructions in BB code with estimated error probability, assuming physical error rate $p=10^{-3}$, where single-qubit Pauli gate and CNOT gate error same as physical error rate. We also assume syndrome measurement and decoding after each logical operation.}
    \label{tab:QLDPCinst}
\end{table*}

\begin{table*}[t]
    \centering
    \begin{tabular}{ p{3.6cm}||p{2cm}|p{2.6cm}|p{4cm}|p{4cm}}
     \hline
     \hline
       Operations & $p=10^{-5}$ Fit by BCG24 & $p=10^{-4}$ & $p=10^{-3}$ & Notes \\
     \hline
     Pauli operators & $10^{-17}$ & $10^{-12}$ & $10^{-7}$ & \\
     \hline
     Automorphism & $10^{-17}$ & $10^{-12}$ & $10^{-7}$ &   \\
     \hline
     ZX-duality & $5*10^{-6}$ & Not-fault-tolerant & Not-fault-tolerant & $132p$ gives a physical error rate higher than the threshold of the code  \\
     \hline
     Measurement-based CNOT[CKBB]&  no-simulation results &  no-simulation results & $10^{-3}$ from Qian Xu &  \\
     \hline
     Measurement-based CNOT[SSIP]&  no-simulation results &  no-simulation results & no-simulation results&  \\
     \hline
     Measurement-based CNOT[mono-layer]&  $ 3*10^{-17}$ & $ 6* 10^{-12}$ & $ 9* 10^{-5}$& Not sure if works for BB+Surface \\
    \end{tabular}
    \caption{Instructions in BB code with estimated error probability, assuming physical error rate $p=10^{-3}$, where single-qubit Pauli gate and CNOT gate error same as physical error rate. We also assume syndrome measurement and decoding after each logical operation.}
    \label{tab:QLDPCinst2}
\end{table*}


\begin{table*}[t]
    \centering
    \begin{tabular}{ p{3.6cm}||p{2cm}|p{2.6cm}|p{4cm}|p{4cm}}
     \hline
     \hline
       Operations & Ancillary qubits & Circuit Depth & Logical error probability & logical clock rate \\
     \hline
     Pauli operators & null & 1 gate time (parallelism 12) & idling error $10^{-7}$ &  \\
     \hline
     magic state  & null & varied gate time& idling error $10^{-7}$ &  \\
     \hline
    \end{tabular}
    \caption{Instructions in surface code with estimated error probability, assuming physical error rate $p=10^{-3}$.}
    \label{tab:surinst}
\end{table*}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figs/adjmatrix.pdf}
    \caption{Automorphism rounds required between the movement of logical qubits X/Z}
            \label{fig:adjmatrix}
\end{figure}

\subsection{Logical qubit mapper and Fault-tolerant compiler}
We will need to design a logical qubit mapper in the circuits. Based on the DAG, we need to track if a qubit is in Memory, where in Memory, or where in Surface code. Notice that this could be high, but in this work, we will \textbf{not} focus on the routing optimization problem. 

Instead, we assume the ancillary block is linked to the first logical qubit, labeled as $k=0$ ($\alpha=0$), where $k$ is a logical qubit label and $\alpha$ is the monomial corresponding to 

As introduced in the ancilla instructions, the fault-tolerant compiler could generate the minimum-round automorphism operations required for a specific permutation of physical qubits. The logical qubit mapper then will update the index of each logical qubit according to every automorphism/ZX duality gate is applied, and synthesize next-round automorphism gates according to the current logical qubit distribution topology.

The number of automorphism gates needed in the gross code are numerically searched and listed in Figure~\ref{fig:stepx} and Figure~\ref{fig:stepz}.


